Sub-annular structure in black hole image from gravitational refraction

The images of supermassive black holes captured by the Event Horizon Telescope (EHT) collaboration have allowed us to have access to the physical processes that occur in the vicinity of the event horizons of these objects. This has enabled us to learn more about the state of rotation of black holes, about the formation of relativistic jets in their vicinity, about the magnetic field in the regions close to them, and even about the existence of the photon ring. Furthermore, black hole imaging gives rise to a new way of testing general relativity in the strong field regime. This has initiated a line of research aimed at probing different physical scenarios. While many scenarios have been proposed in the literature that yield distortion effects that would be a priori detectable at the resolution achieved by future EHT observations, the vast majority of those scenarios involve strange objects or exotic matter content. Here, we consider a less heterodox scenario which, involving non-exotic matter, in the sense that it satisfies all energy conditions and is dynamically stable, also leads to a deformation of the black hole shadow. We consider a specific concentration of non-emitting, relativistic matter of zero optical depth forming a bubble around the black hole. Due to gravitational refraction, such a self-interacting -- dark -- matter concentration may produce sub-annular images, i.e. subleading images inside the photon ring. We calculate the ray tracing in the space-time geometry produced by such a matter configuration and obtain the corresponding black hole images. While for concreteness we restrict our analysis to a specific matter distribution, modeling the bubble as a thin-shell, effects qualitatively similar to those described here are expected to occur for more general density profiles.

==> packages.tex <==
%\usepackage[spanish, es-nosectiondot]{babel} % Soporte idioma español. El paquete babel spanish introduce un punto en la numeración de las secciones (no así babel english), e.g. 3.1. [Section_name]. El parámetro es-nosectiondot sirve para sacarlo, e.g. 3.1 [Section_name]. 
\usepackage[english]{babel}
\usepackage[utf8]{inputenc}

\usepackage{indentfirst} %Paquete necesario para que haya 
\setlength{\parindent}{1.25em} %Cantidad de indentaciónindentación por default
\setlength{\parskip}{0.75em} %Espacio entre parrafos

\usepackage[top=3cm,bottom=3cm, left=2cm, right=2cm]{geometry}

\usepackage{hyperref} %Para que las referencias sean hipervinculos
\hypersetup{
            colorlinks=true,
            linkcolor=blue,
            urlcolor=violet,
            citecolor=violet,
            }

\usepackage{subfiles}

\usepackage{amsmath} % Necesario para estructuras donde escribir ecuaciones, e.g. align
\usepackage{amsfonts}

\numberwithin{equation}{section}

%\addto\captionsspanish{% Replace "spanish" with the language you use
%  \renewcommand{\contentsname}%
%    {Índice}%
%} % Reemplaza el título en el table of contents. Esta forma funciona si se usa el paquete 'babel'. En caso de no usar el paquete babel se usa "\renewcommand*\contentsname{whatever}".

\linespread{1.25}
%\usepackage{setspace}
%\onehalfspacing

\usepackage{enumitem} % Necesario para cambiar a bullets los itemize.

\usepackage{graphicx}
\usepackage{float}
\usepackage{subcaption}

\usepackage{esint} % Integrales con sentido de circulación

%\usepackage[inline]{showlabels} % Muestra los labels de forma explícita en el documento para llamarlos fácil. Se comenta en la compilación final

\usepackage{xr} % Paquete necesario para referenciar estructuras de otro capítulo cuando se compilan individualmente.

\usepackage{cite}

\usepackage{xcolor}

\newcommand{\of}[1]{ \! \left( #1 \right ) }
\newcommand{\off}[1]{ \! \left [ #1 \right ] }
\newcommand{\offf}[1]{ \! \left \{ #1 \right \} }
\newcommand{\abs}[1]{ \left | #1 \right | }
\newcommand{\comm}[2]{ \off{#1, #2} }
\newcommand{\acomm}[2]{ \offf{#1, #2} }
\newcommand{\bra}[1]{ \left \langle #1 \right | }
\newcommand{\ket}[1]{ \left | #1 \right \rangle }
\newcommand{\inprod}[2]{ \langle #1 | #2 \rangle }
\newcommand{\mv}[1]{ \langle #1 \rangle }
\newcommand{\tr}{ \text{Tr} }
\newcommand{\re}{ \text{Re} }
\newcommand{\im}{ \text{Im} }
\newcommand{\bx}{ \mathbf x }
